Reinforcement Learning with Heterogeneous Data: Estimation and Inference

Reinforcement Learning (RL) has the promise of providing data-driven support for decision-making in a wide range of problems in healthcare, education, business, and other domains. Classical RL methods focus on the mean of the total return and, thus, may provide misleading results in the setting of the heterogeneous populations that commonly underlie large-scale datasets. We introduce the K-Heterogeneous Markov Decision Process (K-Hetero MDP) to address sequential decision problems with population heterogeneity. We propose the Auto-Clustered Policy Evaluation (ACPE) for estimating the value of a given policy, and the Auto-Clustered Policy Iteration (ACPI) for estimating the optimal policy in a given policy class. Our auto-clustered algorithms can automatically detect and identify homogeneous sub-populations, while estimating the Q function and the optimal policy for each sub-population. We establish convergence rates and construct confidence intervals for the estimators obtained by the ACPE and ACPI. We present simulations to support our theoretical findings, and we conduct an empirical study on the standard MIMIC-III dataset. The latter analysis shows evidence of value heterogeneity and confirms the advantages of our new method.

==> 1-nota.tex <==
Let lowercase letter $x$, boldface letter $\bx$, and boldface capital letter $\bX$ represent scalar, vector, and matrix, respectively.
%We use the notation $[N]$ to refer to the positive integer set $\braces{1, \ldots, N}$ for $N \in \ZZ_+$.
For any matrix $\bX$,  we use $\bx_{i \cdot}$, $\bx_{\cdot j}$, and $x_{ij}$ to refer to its $i$-th row, $j$-th column, and $ij$-th entry, respectively.
All vectors are column vectors and row vectors are written as $\bx^\top$ for any vector $\bx$.

We write $\sigma_i$ be the $i$-th largest square root of eigenvalues of $\bX^\top \bX$, which are called the singular values of $\bX$.
Then $\sigma_1$ is the largest in absolute value among $\sigma_i$.
%We use the following matrix norms:
%maximum norm $\norm{\bX}_{max} \defeq \underset{ij}{\max} \; \lvert x_{ij} \rvert$,
%$\ell_1$-norm $\norm{\bX}_1 \defeq \underset{j}{\max} \sum_{i} \lvert x_{ij} \rvert$,
%$\ell_{\infty}$-norm $\norm{\bX}_{\infty} \defeq \underset{i}{\max} \; \sum_{j} \lvert x_{ij} \rvert$,
We denote the matrix $\ell_2$-norm as $\norm{\bX}_2 \defeq \sigma_1$ and max norm as $\norm{\bX}_{\max} \defeq \underset{i,j}{\max} \abs{x_{ij}}$
%$(2,\ell_\infty)$-norm $\norm{\bX}_{(2,\ell_\infty)} \defeq \underset{\norm{\ba}_2=1}{\max} \norm{\bX\ba}_\infty = \underset{i}{\max} \norm{\bx_{i \cdot}}_2$.
When $\bX$ is a square matrix, we denote by $\Tr \paran{\bX}$, $\lambda_{max} \paran{\bX}$, and $\lambda_{min} \paran{\bX}$ the trace, maximum and minimum eigenvalues of $\bX$, respectively.
%In addition, define projection matrices $\bP_X^\perp = \bI - \bP_X$ and $\bP_X = \bX \paran{\bX^\top\bX}^{-1} \bX^\top$; when $\bX^\top\bX$ is not inversible, then $\paran{\bX^\top\bX}^{-1}$ is replaced by the Moore-Penrose generalized inverse of $\bX^\top\bX$.
We denote $\mat{\bx}$ as the matricization of a vector $\bx$ and $\vect{\bX}$ as the vectorization of a matrix $\bX$.

Notation $\bbone$ represents a vector or a matrix of all ones of proper size.
We write by $a \asymp b$ when $a = \bigO{b}$ and $b = \bigO{a}$.
We let $C, c, C_0, c_0, \ldots$ denote generic constants, where the uppercase and lowercase letters represent large and small constants, respectively. The actual values of these generic constants may vary from time to time.

The rest of this paper is organized as follows.
In Section \ref{sec:model}, we introduce estimation method.
In Section \ref{sec:theory}, we develop the theoretical results.
In Section \ref{sec:simu}, we study the finite sample performance of our estimation via simulation.
Section \ref{sec:appl} provides an empirical study.
Section \ref{sec:summ} concludes.
All proofs and technique lemmas are relegate to the supplementary appendix (See Appendix \ref{sec:proof}).

==> 99-proof-A.tex <==

%!TEX root = 0-main.tex

\section{Proofs:MDP properties}

\noindent\textbf{Proof of Lemma \ref{lemma:q-bellman-cons-2}.}
\begin{proof}
    Under the assumptions of TH Markov and CMI, we have
    \begin{equation*}
        Q_i\paran{\pi, \bx, a} = r_i\paran{\bx, a} + \gamma\;\EE\brackets{ \E{ \underset{t\ge 0}{\sum} \gamma^t  Y_{i,t+1} \big| \bX_{i,1}, A_{i,1}} \bigg| \bX_{i,0} = \bx, A_{i,0} = a},
    \end{equation*}
    where $r_i(\bx, a) = \EE[Y_{i,t}|\bX_{i,t}=\bx, A_{i,t}=a]$.
    Thus, the $Q$ function satisfies the following Bellman consistency equation:
    \begin{equation}  \label{eqn:q-bellman-cons}
        \begin{aligned}
            Q_i(\pi, \bx, a) & = r_i(\bx, a) + \gamma\;\EE\brackets{ Q_i\paran{\pi, \bX_{0,1}, A_{0,1}} \bigg| \bX_{0,0} = \bx, A_{0,0} = a}  \\
            & = r_i(\bx, a) + \gamma\; \sum_{a'\in\calA} \int_{\bx'} Q_i(\pi, \bx', a') \pi(a' | \bx') \Pr{}_i(d\bx'|\bx, a).
        \end{aligned}
    \end{equation}

    We further obtain a first moment condition of the $Q$ function:
    \begin{equation*}
        \E{ Y_{i,t} + \gamma \sum_{a'\in\calA} Q_i(\pi, \bX_{i,t+1}, a' ) \pi(a'|\bX_{i,t+1}) - Q_i(\pi, \bX_{i,t}, A_{i,t}) \bigg | \bX_{i,t}, A_{i,t}} = 0.
    \end{equation*}
\end{proof}
